A Tool for Estimating Success Rates of Raycasting-Based Object Selection in Virtual Reality

As XR devices become widespread, 3D interaction has become commonplace, and UI developers are increasingly required to consider usability to deliver better user experiences. The HCI community has long studied target-pointing performance, and research on 3D environments has progressed substantially. However, for practitioners to directly leverage research findings in UI improvements, practical tools are needed. To bridge this gap between research and development in VR systems, we propose a system that estimates object selection success rates within a development tool (Unity). In this paper, we validate the underlying theory, describe the tool's functions, and report feedback from VR developers who tried the tool to assess its usefulness.

==> acmart-preload-hook.tex <==
% acmart-preload-hook.tex  (safe version: no \makeatletter, no @-macros)

\AtBeginDocument{%

  % 「Manuscript submitted to ACM」をフッターから消す
  \expandafter\gdef\csname @acmArticle@footer@text\endcsname{}
  \expandafter\gdef\csname @acmArticle@footer\endcsname{}
  \expandafter\gdef\csname @ACM@manuscript@foot\endcsname{}
  \expandafter\gdef\csname @ACM@manuscript@head\endcsname{}


  % ACM Reference Format を出さない
  \settopmatter{printacmref=false}

  % Permission の長文を潰して © 行だけにする
  \setcopyright{rightsretained}
  \copyrightyear{2025}
  \acmYear{2025}
  \renewcommand\footnotetextcopyrightpermission[1]{%
    \footnotetext{© 2025 Copyright held by the owner/author(s).}%
  }

  % 「Manuscript submitted to ACM」を消したい場合（@ を直接使わず csname で叩く）
  \csname @ACM@manuscriptfalse\endcsname
}

